Frequency-Selective Beamforming Cancellation Design for Millimeter-Wave Full-Duplex

The wide bandwidths offered at millimeter-wave (mmWave) frequencies have made them an attractive choice for future wireless communication systems. Recent works have presented beamforming strategies for enabling in-band full-duplex (FD) capability at mmWave even under the constraints of hybrid beamforming, extending the exciting possibilities of next-generation wireless. Existing mmWave FD designs, however, do not consider frequency-selective mmWave channels. Wideband communication at mmWave suggests that frequency-selectivity will likely be of concern since communication channels will be on the order of hundreds of megahertz or more. This has motivated the work of this paper, in which we present a frequency-selective beamforming design to enable practical wideband mmWave FD applications. In our designs, we account for the challenges associated with hybrid analog/digital beamforming such as phase shifter resolution, a desirably low number of radio frequency (RF) chains, and the frequency-flat nature of analog beamformers. We use simulation to validate our work, which indicates that spectral efficiency gains can be achieved with our design by enabling simultaneous transmission and reception in-band.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> sec-acknowledgement.tex <==
\section*{Acknowledgments}

We thank Arun Ghosh, Tom Novlan, Milap Majmundar, and Salam Akoum from AT\&T Labs for their insights.

==> sec-system-model-v2.tex <==
\section{System Model} \label{sec:system-model}

In our design, we consider the \mmwave network exhibited in \figref{fig:network}. We assume node $i$ is a \fd transceiver capable of simultaneously realizing independent transmit and receive beamformers, while nodes $j$ and $k$ are \hd devices. 

Let there be $\Nt\node{m}$ $\left(\Nr\node{m}\right)$ be the number of transmit (receive) antennas at node $m \in \{i,j,k\}$. Similarly, let $\Nrftx\node{m}$ $\left(\Nrfrx\node{m}\right)$ be the number of \rf chains at the transmitter (receiver) of node $m \in \{i,j,k\}$.

Let all channels be frequency-selective over the band of interest. Being frequency-selective, assume the (maximum) channel length is $D$, and $d \in \{ 0,\dots,D-1 \}$ represents the channel tap index (in time). We assume a scheme such as \gls{ofdm} is used for sufficiently transforming the frequency-selective wideband channel into a bank of $U$ frequency-flat subchannels. Let $u \in \{0,\dots,U-1\}$ denote the subcarrier index. Let $\channelfd_{m,n}[u]$ be the frequency-flat \mimo channel matrix for subcarrier $u$ where $m,n \in \{i,j,k\}$.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.27\textwidth]{fig/ijk_dl_ul_si_labels.pdf}
	\caption{A \fd node $(i)$ suffering from \si as it simultaneously transmits to $(j)$ and receives from $(k)$.}
	\label{fig:network}
\end{figure}

We assume node $i$ employs fully-connected hybrid beamforming at its precoder and combiner.
Let $\prebbfd\node{i}[u]$ $\left(\combbfd\node{i}[u]\right)$ be the baseband precoding (combining) matrix at $i$ for subcarrier $u$. Unlike the baseband beamformers, the \rf beamformer is not frequency-selective, but rather frequency-flat and is not indexed per subcarrier. This fact will impact our design in Section~\ref{sec:bfc}. Let $\prerffd\node{i}$ $\left(\comrffd\node{i}\right)$ be the \rf precoding (combining) matrix at $i$. We impose a \gls{ca} constraint on the entries of the \rf beamformers representing the fact that they have phase control and no amplitude control. Further, we assume that the phase shifters have some finite resolution.

% We assume $j$ and $k$ can perfectly realize a fully-digital beamformer, perhaps in a hybrid fashion (e.g., using \cite{wei-yu}). 
Let $\prebbfd\node{j}[u]$ and $\prebbfd\node{k}[u]$ be the baseband precoders at $j$ and $k$, respectively, for subcarrier $u$. Let $\combbfd\node{j}[u]$ and $\combbfd\node{k}[u]$ be the digital combiners at $j$ and $k$, respectively, for subcarrier $u$.
Let $\prerffd\node{j}$ and $\prerffd\node{k}$ be the \rf precoders at $j$ and $k$, respectively. Let $\comrffd\node{j}$ and $\comrffd\node{k}$ be the \rf combiners at $j$ and $k$, respectively.

Let $\symbvec\node{m}[u] \sim \cgauss{\mat{0}}{\mat{R_s}}$ be the $\Ns\node{m} \times 1$ symbol vector transmitted on subcarrier $u$ intended for node $m \in \{i,j,k\}$, where we have assumed each subcarrier is transmitted with the same number of streams. It is assumed that the devices have proper support for the number of streams being communicated (i.e., sufficient number of \rf chains).

Let $\noisevec\node{m}[u] \sim \cgauss{\mat{0}}{\mat{R_n}}$ be a noise vector received by the receive array at node $m$ on subcarrier $u$, where we have assumed a common (and frequency-flat) noise covariance matrix. Let $\mat{R_n} = \sigma^2_n \mat{I}$ and $\mat{R_s} = \mat{I}$.

We define the link \gls{snr} (without beamforming) from node $m$ to node $n$ as 
\begin{align}
\snr_{m,n} = \frac{\Pt\node{m} \ G^2_{m,n}}{\sigma^2_n}
\end{align}
where $\Pt\node{m}$ is the transmit power of $m$ and $G_{m,n}$ is the large-scale gain of the channel between $m$ and $n$. Note that we have assumed a frequency-flat transmit power and large-scale gain.

Let us consider the network in \figref{fig:network} where $i$ is transmitting to $j$ while $i$ is receiving from $k$. The familiar \mimo formulation on a per subcarrier basis gives us an estimated received symbol as
\begin{align}
\rxvec\node{i}[u] &= \sqrt{\snr_{ki}} \ \combbfd\ctransnode{i}[u] \comrf\ctransnode{i} \channel_{ki}[u] \pre\node{k}[u] \symbvec\node{i}[u] \label{eq:term-desired} \\
&+ \sqrt{\snr_{ii}[u]} \ \combb\ctransnode{i}[u] \comrf\ctransnode{i} \channel_{ii}[u] \prerf\node{i} \prebb\node{i}[u] \symbvec\node{j}[u] \label{eq:term-si} \\
&+ \combb\ctransnode{i}[u] \comrf\ctransnode{i} \noisevec\node{i}[u] \label{eq:term-noise}
\end{align}
where \eqref{eq:term-desired} is the desired term, \eqref{eq:term-si} is the resulting \si term, and \eqref{eq:term-noise} is the resulting noise term. As indicated by \eqref{eq:term-si}, the transmitted signal from $(i)$ intended for $(j)$ traverses through the \si channel $\channel_{ii}$ and is received by the combiner at $(i)$ being used for reception from $(k)$. 

The estimated receive symbol at $(j)$ from $(i)$ is
\begin{align}
\rxvec\node{j}[u] &= \sqrt{\snr_{ij}[u]} \ \com\ctransnode{j}[u] \channel_{ij}[u] \prerf\node{i} \prebb\node{i}[u] \symbvec\node{j}[u] \\ &+ \com\ctransnode{j}[u] \noisevec\node{j}[u] \label{eq:term-j},
\end{align}
where $(j)$ does not encounter any \si since it is a \hd device. Additionally, we assume that there is no adjacent user interference between $(j)$ and $(k)$. We justify this assumption with the high path loss and directionality of transmission and reception at \mmwave.

For the sake of analysis, we impose the following power constraints and normalizations. The baseband precoder at $m$ performs uniform power allocation across streams and are normalized such that the Frobenius norm of each beamformer (column) in the matrix is $\sqrt{\Nt\node{m}}$. The \rf precoding matrix at $i$ is normalized such that its columns have unit norm. The \rf combining matrix at $i$ is normalized such that its columns have norm $\Nr$, though this is of less importance since the combiner is acting on the desired signal plus noise and interference.

As a worst-case in analysis, we consider interference as noise and ignore adjacent user interference, as evidenced by \eqref{eq:term-j}. We justify this assumption with the high path loss and directionality of transmission and reception at \mmwave.

For evaluating our designs, we use spectral efficiency, which, given our symbol and noise distributions and treating interference as noise, is the so-called Gaussian mutual information \cite{heath_lozano}. More concretely, the spectral efficiency (in bps/Hz) of communication from $i$ to $j$ is as follows.

%  R = log2 det [ I  + W' H F Rs F' H' W (W' Rn W + W' Q Q' W)^(-1) ]

We define the noise-plus-self-interference term at $i$ as
\begin{align}
\mat{Q}\node{i} = \mat{R_n} + \channel_{ii} \prerf\node{i} \prebb\node{i} \mat{R_s}  \prebb\ctransnode{i} \prerf\ctransnode{i} \channel_{ii}\ctrans .
\end{align}

At $j$, being a \hd device, there is no self-interference, resulting in simply
\begin{align}
\mat{Q}\node{j} = \mat{R_n} .
\end{align}

The spectral efficiency on the link from $i$ to $j$ is
\begin{align}
R_{ij} = \log_2 \left| \mat{I} + \com\ctransnode{j} \channel_{ij} \prerf\node{i} \prebb\node{i} \mat{R_s} \prebb\ctransnode{i} \prerf\ctransnode{i} \channel_{ij}\ctrans \com\node{j} \left( \com\ctransnode{j} \mat{R_n} \com\node{j} \right)^{-1} \right|
\end{align}

The spectral efficiency on the link from $k$ to $i$ is
\begin{align}
R_{ki} =& \log_2 \Bigg| \mat{I} + \combb\ctransnode{i} \comrf\ctransnode{i} \channel_{ki} \pre\node{k} \mat{R_s} \pre\ctransnode{k} \channel_{ki}\ctrans \comrf\node{i} \combb\node{i} \nonumber \\ &\times \left( \combb\ctransnode{i} \comrf\ctransnode{i} \left( \mat{R_n} + \channel_{ii} \prerf\node{i} \prebb\node{i} \mat{R_s}  \prebb\ctransnode{i} \prerf\ctransnode{i} \channel_{ii}\ctrans \right) \comrf\node{i} \combb\node{i} \right)^{-1} \Bigg|
\end{align}

The spectral efficiency on the link from $k$ to $i$ is
\begin{align}
R_{ki} =& \log_2 \Bigg| \mat{I} + \combb\ctransnode{i} \comrf\ctransnode{i} \channel_{ki} \pre\node{k} \mat{R_s} \pre\ctransnode{k} \channel_{ki}\ctrans \comrf\node{i} \combb\node{i} 
%\nonumber \\ &\times 
\left( \combb\ctransnode{i} \comrf\ctransnode{i} \mat{Q}\node{i} \comrf\node{i} \combb\node{i} \right)^{-1} \Bigg|
\end{align}

For the desired link channels, $\channel_{ij}$ and $\channel_{ki}$, we assume sufficient far-field conditions have been met. 
We employ the extended Saleh-Valenzuela \mmwave channel representation as shown in \eqref{eq:clustered-channel-model}. In this model, an $\Nr\times\Nt$ channel is the sum of the contributions from \numclust scattering clusters, each of which contributes \numrays propagation paths \cite{Mendez-Rial_Rusu_Gonzalez-Prelcic_Alkhateeb_Heath_2016}. 
%Such a channel results in a sparse channel, being the combination of a discrete number of paths that propagate from the transmit array and impinge the receive array.
\begin{equation} \label{eq:clustered-channel-model}
\mat{H} = \sqrt{\frac{\Nt \Nr}{\numrays \numclust}} \sum_{m=1}^{\numclust} \sum_{n=1}^{\numrays} \beta_{m,n} \rxresponsevector(\aoa_{m,n}) \txresponsevector\ctrans(\aod_{m,n})
\end{equation}
In \eqref{eq:clustered-channel-model}, $\rxresponsevector(\aoa_{m,n})$ and $\txresponsevector(\aod_{m,n})$ are the antenna array responses 
at the receiver and transmitter, respectively, for ray $n$ within cluster $m$ which has some \gls{aoa}, $\aoa_{m,n}$, and \gls{aod}, $\aod_{m,n}$. Each ray has a random gain $\beta_{m,n} \sim \cgauss{0}{1}$. The coefficient outside the summations is used to ensure that $\ev{ \frobeniustwo{ \mat{H} }} = \Nt\Nr$. Note that we have considered a single angular dimension (e.g., azimuth) for the \glspl{aoa} and \glspl{aod} for simplicity and to agree with our use of \glspl{ula} in simulation.

When $(i)$ transmits to $(j)$ while receiving from $(k)$, there will almost certainly be some undesired leakage from the transmit array to the receive array that corrupts the desired receive signal. The strength of this leakage is a function of the  precoder at $(i)$, the combiner at $(i)$, and the channel between them. The transmit and receive arrays at $(i)$ will be relatively close together, meaning the far-field condition is not met and near-field effects must be considered. Unfortunately, the \mmwave \si channel is much less understood since research and measurements at \mmwave have primarily focused on more practical far-field scenarios. Therefore, we have turned to one of the few attempts at characterizing the \mmwave \si channel \cite{Satyanarayana_El-Hajjar_Kuo_Mourad_Hanzo_2019}, where it is decomposed in a Rician fashion containing a near-field \gls{los} component and a far-field component stemming from \gls{nlos} reflections. Explicitly, we model the \si as 
\input{eq-si-channel-rice.tex}
where $\kappa$ is the Rician factor. The entries of the \gls{los} contribution are modeled as \cite{spherical-wave-mimo}
\input{eq-si-channel-los.tex}
where $\rho$ is a normalization constant such that $\ev{\frobeniustwo{\channel_{ii}}} = \Nt\Nr$ and $r_{m,n}$ is the distance from the $m$th element of the transmit array to the $n$th element of the receive array. For the \gls{nlos} \si channel, we use the model in \eqref{eq:clustered-channel-model}.\

---

The channel is $D$ taps in time and $d = 0,\dots,D-1$ is the tap index. The channel matrix between a one node's transmit array and another node's receive array can be written as
\begin{align}
\channel[d] = \sqrt{\frac{\Nt \Nr}{\numrays \numclust}} \sum_{m=1}^{\numclust} \sum_{n=1}^{\numrays} \beta_{m,n} \rxresponsevector(\aoa_{m,n}) \txresponsevector\ctrans(\aod_{m,n})
\end{align}
We assume \gls{ofdm} (with a sufficient cyclic prefix) is used such that the frequency-selective wideband channel can be decomposed into a bank of parallel frequency-flat narrowband subchannels.

Having an effective circularly-convolved channel, we take a $U$-point \gls{dft} of the channel matrices across time to get \mimo channels across subcarriers, which are narrowband and thus constant over time.
\begin{align}
\matfd{H}[u] = \sum_{d=0}^{D-1} \channel[d] \ e^{-\j \frac{2 \pi u d}{U}}
\end{align}

In particular, we are concerned with the desired channels $\channelfd_{ij}[u]$ and $\channelfd_{ki}[u]$. Taking the \gls{svd} of each, we get
\begin{align}
\channelfd_{ij}[u] = \svdfd{\channelfd_{ij}}{[u]} \\
\channelfd_{ki}[u] = \svdfd{\channelfd_{ki}}{[u]}
\end{align}

The effective precoder at node $m$ on subcarrier $u$ is $\pre\node{m}[u] = \prerf\node{m} \prebb\node{m}[u]$.

The effective combiner at node $m$ on subcarrier $u$ is $\com\node{m}[u] = \comrf\node{m} \combb\node{m}[u]$.

Since the \rf precoder and combiner are frequency-flat, they are chosen based on what?

\begin{align}
\max_{\prerf \in \prerfcb} \ \left\{ \max_{\{\prebb[u]\}} \ R_{ij}\left(\{\prebb[u]\},\prerf\right) \ \st \text{TBD power constraint}  \right\} \label{eq:max-spec-eff}
\end{align}
---

The frequency-domain channel matrix on subcarrier $u$ is
\begin{align}
\channelfd[u] = \svdfd{\channelfd}{[u]}
\end{align}

Considering the following and taking its \gls{svd} we get,
\begin{align}
\matfd{\Sigma}_{\channelfd}[u] \ \matfd{V}\ctrans_{\channelfd}[u] \prerf \left(\prerf\ctrans \prerf \right)^{-1/2} &= \bar{\channelfd} \\ &= \svdfd{\bar{\channelfd}}{[u]}
\end{align}

Then the optimal digital precoder for \eqref{eq:max-spec-eff} is
\begin{align}
\prebb\opt[u] = \left(\prerf\ctrans \prerf \right)^{-1/2} \left[ \matfd{V}_{\bar{\channelfd}} [u] \right]_{:,1:\Ns} \mat{\Lambda}[u]
\end{align}
where $\mat{\Lambda}[u]$ is an $\Ns \times \Ns$ waterfilling power allocation diagonal matrix. If equal power across all streams of all subcarriers, $\mat{\Lambda}[u] = \mat{I}$.

This indicates that \eqref{eq:max-spec-eff} is now only a function of $\prerf$. From here, we can simply exhaustively search over the codebook to find the analog beamformer maximizing \eqref{eq:max-spec-eff}.

---
\newpage
We assume perfect CSI of $\channel_{ij}$, $\channel_{ki}$, and $\channel_{ii}$.

We fix $\pre\node{k}$ and $\com\node{j}$ to be the eigen-beamformers of their respective channels.

We fix $\prerf\node{i}$ and $\comrf\node{i}$ to be the analog result of hybrid decomposition of the eigen-beamformers of their respective channels.

The spectral efficiency of the link from $i$ to $j$ is then a function only of the baseband precoder at $i$ and is written as
\begin{align}
R_{ij}\left(\prebb\node{i}\right) = \log_2 \left| \mat{I} + \com\ctransnode{j} \channel_{ij} \prerf\node{i} \prebb\node{i} \mat{R_s} \prebb\ctransnode{i} \prerf\ctransnode{i} \channel_{ij}\ctrans \com\node{j} \left( \com\ctransnode{j} \mat{R_n} \com\node{j} \right)^{-1} \right|
\end{align}

The spectral efficiency of the link from $k$ to $i$ is a function of the baseband precoder at $i$ and the baseband combiner at $i$ and is written as
\begin{align}
R_{ki}\left(\prebb\node{i},\combb\node{i}\right) =& \log_2 \Bigg| \mat{I} + \combb\ctransnode{i} \comrf\ctransnode{i} \channel_{ki} \pre\node{k} \mat{R_s} \pre\ctransnode{k} \channel_{ki}\ctrans \comrf\node{i} \combb\node{i} \nonumber \\ &\times \left( \combb\ctransnode{i} \comrf\ctransnode{i} \left( \mat{R_n} + \channel_{ii} \prerf\node{i} \prebb\node{i} \mat{R_s}  \prebb\ctransnode{i} \prerf\ctransnode{i} \channel_{ii}\ctrans \right) \comrf\node{i} \combb\node{i} \right)^{-1} \Bigg|
\end{align}

We take an iterative approach to designing the digital precoder and digital combiner at $(i)$.

Let $t$ be the iteration index. 

We initialize $\prebb\node{i}(0)$ and $\combb\node{i}(0)$ as the digital result of hybrid decomposition of the eigen-beamformers of their respective channels.

We first solve for the baseband precoder that maximizes the sum rate.
\begin{align}
\prebb\node{i}(t+1) =& \arg \max_{\prebb} \left\{ \ R_{ij}\left(\prebb\node{i}\right) + R_{ki}\left(\prebb\node{i},\combb\node{i}(t)\right) \right\} \\
&\st \ \frobeniustwo{\prebb\node{i}} \leq \Ns \Nt
\end{align}

Using this choice of $\prebb\node{i}(t+1)$, we solve for the baseband combiner that maximizes the sum rate.
\begin{align}
\combb\node{i}(t+1) =& \arg \max_{\combb} \left\{ \ R_{ij}\left(\prebb\node{i}(t+1)\right) + R_{ki}\left(\prebb\node{i}(t+1),\combb\node{i}\right) \right\} 
% \\ &\st \ \frobeniustwo{\prebb\node{i}} = \Ns \Nt
\end{align}
We iterate between these for a maximum number of iterations or until a convergence criterion is met.

\newpage

Grouping constant terms, we define
\begin{align}
\mat{A} &= \com\ctransnode{j} \channel_{ij} \prerf\node{i} \\
\mat{B} &= \left( \com\ctransnode{j} \mat{R_n} \com\node{j} \right)^{-1}
\end{align}
This gives us the simplified expression
\begin{align}
R_{ij}\left(\prebb\node{i}\right) = \log_2 \left| \mat{I} + \mat{A} \prebb\node{i} \mat{R_s} \prebb\ctransnode{i} \mat{A}\ctrans \mat{B} \right|
\end{align}

Similarly, grouping constant terms, we define
\begin{align}
\mat{C} &= \comrf\ctransnode{i} \channel_{ki} \pre\node{k} \mat{R_s} \pre\ctransnode{k} \channel_{ki}\ctrans \comrf\node{i} \\
\mat{D} &= \channel_{ii} \prerf\node{i}
\end{align}
This gives us the simplified expression 
\begin{align}
R_{ki}\left(\prebb\node{i},\combb\node{i}\right) =& \log_2 \Bigg| \mat{I} + \combb\ctransnode{i} \mat{C} \combb\node{i} \left( \combb\ctransnode{i} \comrf\ctransnode{i} \left( \mat{R_n} + \mat{D} \prebb\node{i} \mat{R_s}  \prebb\ctransnode{i} \mat{D}\ctrans \right) \comrf\node{i} \combb\node{i} \right)^{-1} \Bigg|
\end{align}

---



\newpage

==> sec-system-model.tex <==
\section{System Model} \label{sec:system-model}

In our design, we consider the \mmwave network exhibited in \figref{fig:network}. We assume node $i$ is a \fd transceiver capable of simultaneously realizing independent transmit and receive beamformers, while nodes $j$ and $k$ are \hd devices. 

Let there be $\Nt\node{m}$ $\left(\Nr\node{m}\right)$ be the number of transmit (receive) antennas at node $m \in \{i,j,k\}$. Similarly, let $\Nrftx\node{m}$ $\left(\Nrfrx\node{m}\right)$ be the number of \rf chains at the transmitter (receiver) of node $m \in \{i,j,k\}$.

Let all channels be frequency-selective over the band of interest. Being frequency-selective, assume the (maximum) channel length is $D$, and $d \in \{ 0,\dots,D-1 \}$ represents the channel tap index (in time). We assume a scheme such as \gls{ofdm} is used for sufficiently transforming the frequency-selective wideband channel into a series of $U$ frequency-flat subchannels. Let $u \in \{0,\dots,U-1\}$ denote the subcarrier index. Let $\channelfd_{m,n}[u]$ be the frequency-flat \mimo channel matrix for subcarrier $u$ where $m,n \in \{i,j,k\}$.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.27\textwidth]{fig/ijk_dl_ul_si_labels.pdf}
	\caption{A \fd node $(i)$ suffering from \si as it simultaneously transmits to $(j)$ and receives from $(k)$.}
	\label{fig:network}
\end{figure}

We assume node $i$ employs fully-connected hybrid beamforming at its precoder and combiner.
Let $\prebb\node{i}[u]$ $\left(\combb\node{i}[u]\right)$ be the baseband precoding (combining) matrix at $i$ for subcarrier $u$. Unlike the baseband beamformers, the \rf beamformers are not frequency-selective, but rather frequency-flat and are not indexed per subcarrier. This fact will impact our design in Section~\ref{sec:bfc}. Let $\prerf\node{i}$ $\left(\comrf\node{i}\right)$ be the \rf precoding (combining) matrix at $i$. We impose a \gls{ca} constraint on the entries of the \rf beamformers representing the fact that they have phase control and no amplitude control. Further, we assume that the phase shifters have a finite resolution.

We assume $j$ and $k$ can perfectly realize a fully-digital beamformer, perhaps in a hybrid fashion (e.g., using \cite{wei-yu}). Let $\pre\node{j}[u]$ and $\pre\node{k}[u]$ be the effective fully-digital precoders at $j$ and $k$, respectively, for subcarrier $[u]$. Let $\com\node{j}[u]$ and $\com\node{k}[u]$ be the effective fully-digital combiners at $j$ and $k$, respectively, for subcarrier $u$.

Let $\symbvec\node{m}[u] \sim \cgauss{\mat{0}}{\mat{R_s}}$ be the $\Ns\node{m} \times 1$ symbol vector transmitted on subcarrier $u$ intended for node $m \in \{i,j,k\}$, where we have assumed each subcarrier is transmitted with the same number of streams. It is assumed that the devices have proper support for the number of streams being communicated (i.e., sufficient number of \rf chains).

Let $\noisevec\node{m}[u] \sim \cgauss{\mat{0}}{\mat{R_n}}$ be a noise vector received by the receive array at node $m$ on subcarrier $u$, where we have assumed a common (and frequency-flat) noise covariance matrix.

Letting $\mat{R_n} = \sigma^2_n \mat{I}$ and $\mat{R_s} = \mat{I}$, we can write the link \gls{snr} (without beamforming) from node $m$ to node $n$ on subcarrier $u$ as 
\begin{align}
\snr_{m,n}[u] = \frac{\Pt\node{m} \ G^2_{m,n}[u]}{\sigma^2_n}
\end{align}
where $\Pt\node{m}$ is the transmit power of $m$ and $G_{m,n}[u]$ is the large-scale gain of the channel between $m$ and $n$ on subcarrier $u$. Note that we have assumed a frequency-flat transmit power.

Let us consider the network in \figref{fig:network} where $i$ is transmitting to $j$ while $i$ is receiving from $k$. The familiar \mimo formulation on a per subcarrier basis gives us an estimated received symbol as
\begin{align}
\rxvec\node{i}[u] &= \sqrt{\snr_{ki}[u]} \ \combb\ctransnode{i}[u] \comrf\ctransnode{i} \channel_{ki}[u] \pre\node{k}[u] \symbvec\node{i}[u] \label{eq:term-desired} \\
&+ \sqrt{\snr_{ii}[u]} \ \combb\ctransnode{i}[u] \comrf\ctransnode{i} \channel_{ii}[u] \prerf\node{i} \prebb\node{i}[u] \symbvec\node{j}[u] \label{eq:term-si} \\
&+ \combb\ctransnode{i}[u] \comrf\ctransnode{i} \noisevec\node{i}[u] \label{eq:term-noise}
\end{align}
where \eqref{eq:term-desired} is the desired term, \eqref{eq:term-si} is the resulting \si term, and \eqref{eq:term-noise} is the resulting noise term. As indicated by \eqref{eq:term-si}, the transmitted signal from $(i)$ intended for $(j)$ traverses through the \si channel $\channel_{ii}$ and is received by the combiner at $(i)$ being used for reception from $(k)$. 

The estimated receive symbol at $(j)$ from $(i)$ is
\begin{align}
\rxvec\node{j}[u] &= \sqrt{\snr_{ij}[u]} \ \com\ctransnode{j}[u] \channel_{ij}[u] \prerf\node{i} \prebb\node{i}[u] \symbvec\node{j}[u] \\ &+ \com\ctransnode{j}[u] \noisevec\node{j}[u] \label{eq:term-j},
\end{align}
where $(j)$ does not encounter any \si since it is a \hd device. Additionally, we assume that there is no adjacent user interference between $(j)$ and $(k)$. We justify this assumption with the high path loss and directionality of transmission and reception at \mmwave.

For the sake of analysis, we impose the following power constraints and normalizations. The baseband precoder at $m$ performs uniform power allocation across streams and are normalized such that the Frobenius norm of each beamformer (column) in the matrix is $\sqrt{\Nt\node{m}}$. The \rf precoding matrix at $i$ is normalized such that its columns have unit norm. The \rf combining matrix at $i$ is normalized such that its columns have norm $\Nr$, though this is of less importance since the combiner is acting on the desired signal plus noise and interference.

As a worst-case in analysis, we consider interference as noise and ignore adjacent user interference, as evidenced by \eqref{eq:term-j}. We justify this assumption with the high path loss and directionality of transmission and reception at \mmwave.

For evaluating our designs, we use spectral efficiency, which, given our symbol and noise distributions and treating interference as noise, is the so-called Gaussian mutual information \cite{heath_lozano}. More concretely, the spectral efficiency (in bps/Hz) of communication from $i$ to $j$ is as follows.

%  R = log2 det [ I  + W' H F Rs F' H' W (W' Rn W + W' Q Q' W)^(-1) ]

We define the noise-plus-self-interference term at $i$ as
\begin{align}
\mat{Q}\node{i} = \mat{R_n} + \channel_{ii} \prerf\node{i} \prebb\node{i} \mat{R_s}  \prebb\ctransnode{i} \prerf\ctransnode{i} \channel_{ii}\ctrans .
\end{align}

At $j$, being a \hd device, there is no self-interference, resulting in simply
\begin{align}
\mat{Q}\node{j} = \mat{R_n} .
\end{align}

The spectral efficiency on the link from $i$ to $j$ is
\begin{align}
R_{ij} = \log_2 \left| \mat{I} + \com\ctransnode{j} \channel_{ij} \prerf\node{i} \prebb\node{i} \mat{R_s} \prebb\ctransnode{i} \prerf\ctransnode{i} \channel_{ij}\ctrans \com\node{j} \left( \com\ctransnode{j} \mat{R_n} \com\node{j} \right)^{-1} \right|
\end{align}

The spectral efficiency on the link from $k$ to $i$ is
\begin{align}
R_{ki} =& \log_2 \Bigg| \mat{I} + \combb\ctransnode{i} \comrf\ctransnode{i} \channel_{ki} \pre\node{k} \mat{R_s} \pre\ctransnode{k} \channel_{ki}\ctrans \comrf\node{i} \combb\node{i} \nonumber \\ &\times \left( \combb\ctransnode{i} \comrf\ctransnode{i} \left( \mat{R_n} + \channel_{ii} \prerf\node{i} \prebb\node{i} \mat{R_s}  \prebb\ctransnode{i} \prerf\ctransnode{i} \channel_{ii}\ctrans \right) \comrf\node{i} \combb\node{i} \right)^{-1} \Bigg|
\end{align}

The spectral efficiency on the link from $k$ to $i$ is
\begin{align}
R_{ki} =& \log_2 \Bigg| \mat{I} + \combb\ctransnode{i} \comrf\ctransnode{i} \channel_{ki} \pre\node{k} \mat{R_s} \pre\ctransnode{k} \channel_{ki}\ctrans \comrf\node{i} \combb\node{i} 
%\nonumber \\ &\times 
\left( \combb\ctransnode{i} \comrf\ctransnode{i} \mat{Q}\node{i} \comrf\node{i} \combb\node{i} \right)^{-1} \Bigg|
\end{align}

For the desired link channels, $\channel_{ij}$ and $\channel_{ki}$, we assume sufficient far-field conditions have been met. 
We employ the extended Saleh-Valenzuela \mmwave channel representation as shown in \eqref{eq:clustered-channel-model}. In this model, an $\Nr\times\Nt$ channel is the sum of the contributions from \numclust scattering clusters, each of which contributes \numrays propagation paths \cite{Mendez-Rial_Rusu_Gonzalez-Prelcic_Alkhateeb_Heath_2016}. 
%Such a channel results in a sparse channel, being the combination of a discrete number of paths that propagate from the transmit array and impinge the receive array.
\begin{equation} \label{eq:clustered-channel-model}
\mat{H} = \sqrt{\frac{\Nt \Nr}{\numrays \numclust}} \sum_{m=1}^{\numclust} \sum_{n=1}^{\numrays} \beta_{m,n} \rxresponsevector(\aoa_{m,n}) \txresponsevector\ctrans(\aod_{m,n})
\end{equation}
In \eqref{eq:clustered-channel-model}, $\rxresponsevector(\aoa_{m,n})$ and $\txresponsevector(\aod_{m,n})$ are the antenna array responses 
at the receiver and transmitter, respectively, for ray $n$ within cluster $m$ which has some \gls{aoa}, $\aoa_{m,n}$, and \gls{aod}, $\aod_{m,n}$. Each ray has a random gain $\beta_{m,n} \sim \cgauss{0}{1}$. The coefficient outside the summations is used to ensure that $\ev{ \frobeniustwo{ \mat{H} }} = \Nt\Nr$. Note that we have considered a single angular dimension (e.g., azimuth) for the \glspl{aoa} and \glspl{aod} for simplicity and to agree with our use of \glspl{ula} in simulation.

When $(i)$ transmits to $(j)$ while receiving from $(k)$, there will almost certainly be some undesired leakage from the transmit array to the receive array that corrupts the desired receive signal. The strength of this leakage is a function of the  precoder at $(i)$, the combiner at $(i)$, and the channel between them. The transmit and receive arrays at $(i)$ will be relatively close together, meaning the far-field condition is not met and near-field effects must be considered. Unfortunately, the \mmwave \si channel is much less understood since research and measurements at \mmwave have primarily focused on more practical far-field scenarios. Therefore, we have turned to one of the few attempts at characterizing the \mmwave \si channel \cite{Satyanarayana_El-Hajjar_Kuo_Mourad_Hanzo_2019}, where it is decomposed in a Rician fashion containing a near-field \gls{los} component and a far-field component stemming from \gls{nlos} reflections. Explicitly, we model the \si as 
\input{eq-si-channel-rice.tex}
where $\kappa$ is the Rician factor. The entries of the \gls{los} contribution are modeled as \cite{spherical-wave-mimo}
\input{eq-si-channel-los.tex}
where $\rho$ is a normalization constant such that $\ev{\frobeniustwo{\channel_{ii}}} = \Nt\Nr$ and $r_{m,n}$ is the distance from the $m$th element of the transmit array to the $n$th element of the receive array. For the \gls{nlos} \si channel, we use the model in \eqref{eq:clustered-channel-model}.\

---

The channel is $D$ taps in time and $d = 0,\dots,D-1$ is the tap index. The channel matrix between a one node's transmit array and another node's receive array can be written as
\begin{align}
\channel[d] = \sqrt{\frac{\Nt \Nr}{\numrays \numclust}} \sum_{m=1}^{\numclust} \sum_{n=1}^{\numrays} \beta_{m,n} \rxresponsevector(\aoa_{m,n}) \txresponsevector\ctrans(\aod_{m,n})
\end{align}
We assume \gls{ofdm} (with a sufficient cyclic prefix) is used such that the frequency-selective wideband channel can be decomposed into a bank of parallel frequency-flat narrowband subchannels.

Having an effective circularly-convolved channel, we take a $U$-point \gls{dft} of the channel matrices across time to get \mimo channels across subcarriers, which are narrowband and thus constant over time.
\begin{align}
\matfd{H}[u] = \sum_{d=0}^{D-1} \channel[d] \ e^{-\j \frac{2 \pi u d}{U}}
\end{align}

In particular, we are concerned with the desired channels $\channelfd_{ij}[u]$ and $\channelfd_{ki}[u]$. Taking the \gls{svd} of each, we get
\begin{align}
\channelfd_{ij}[u] = \svdfd{\channelfd_{ij}}{[u]} \\
\channelfd_{ki}[u] = \svdfd{\channelfd_{ki}}{[u]}
\end{align}

The effective precoder at node $m$ on subcarrier $u$ is $\pre\node{m}[u] = \prerf\node{m} \prebb\node{m}[u]$.

The effective combiner at node $m$ on subcarrier $u$ is $\com\node{m}[u] = \comrf\node{m} \combb\node{m}[u]$.

Since the \rf precoder and combiner are frequency-flat, they are chosen based on what?

\begin{align}
\max_{\prerf \in \prerfcb} \ \left\{ \max_{\{\prebb[u]\}} \ R_{ij}\left(\{\prebb[u]\},\prerf\right) \ \st \text{TBD power constraint}  \right\} \label{eq:max-spec-eff}
\end{align}
---

The frequency-domain channel matrix on subcarrier $u$ is
\begin{align}
\channelfd[u] = \svdfd{\channelfd}{[u]}
\end{align}

Considering the following and taking its \gls{svd} we get,
\begin{align}
\matfd{\Sigma}_{\channelfd}[u] \ \matfd{V}\ctrans_{\channelfd}[u] \prerf \left(\prerf\ctrans \prerf \right)^{-1/2} &= \bar{\channelfd} \\ &= \svdfd{\bar{\channelfd}}{[u]}
\end{align}

Then the optimal digital precoder for \eqref{eq:max-spec-eff} is
\begin{align}
\prebb\opt[u] = \left(\prerf\ctrans \prerf \right)^{-1/2} \left[ \matfd{V}_{\bar{\channelfd}} [u] \right]_{:,1:\Ns} \mat{\Lambda}[u]
\end{align}
where $\mat{\Lambda}[u]$ is an $\Ns \times \Ns$ waterfilling power allocation diagonal matrix. If equal power across all streams of all subcarriers, $\mat{\Lambda}[u] = \mat{I}$.

This indicates that \eqref{eq:max-spec-eff} is now only a function of $\prerf$. From here, we can simply exhaustively search over the codebook to find the analog beamformer maximizing \eqref{eq:max-spec-eff}.

---
\newpage
We assume perfect CSI of $\channel_{ij}$, $\channel_{ki}$, and $\channel_{ii}$.

We fix $\pre\node{k}$ and $\com\node{j}$ to be the eigen-beamformers of their respective channels.

We fix $\prerf\node{i}$ and $\comrf\node{i}$ to be the analog result of hybrid decomposition of the eigen-beamformers of their respective channels.

The spectral efficiency of the link from $i$ to $j$ is then a function only of the baseband precoder at $i$ and is written as
\begin{align}
R_{ij}\left(\prebb\node{i}\right) = \log_2 \left| \mat{I} + \com\ctransnode{j} \channel_{ij} \prerf\node{i} \prebb\node{i} \mat{R_s} \prebb\ctransnode{i} \prerf\ctransnode{i} \channel_{ij}\ctrans \com\node{j} \left( \com\ctransnode{j} \mat{R_n} \com\node{j} \right)^{-1} \right|
\end{align}

The spectral efficiency of the link from $k$ to $i$ is a function of the baseband precoder at $i$ and the baseband combiner at $i$ and is written as
\begin{align}
R_{ki}\left(\prebb\node{i},\combb\node{i}\right) =& \log_2 \Bigg| \mat{I} + \combb\ctransnode{i} \comrf\ctransnode{i} \channel_{ki} \pre\node{k} \mat{R_s} \pre\ctransnode{k} \channel_{ki}\ctrans \comrf\node{i} \combb\node{i} \nonumber \\ &\times \left( \combb\ctransnode{i} \comrf\ctransnode{i} \left( \mat{R_n} + \channel_{ii} \prerf\node{i} \prebb\node{i} \mat{R_s}  \prebb\ctransnode{i} \prerf\ctransnode{i} \channel_{ii}\ctrans \right) \comrf\node{i} \combb\node{i} \right)^{-1} \Bigg|
\end{align}

We take an iterative approach to designing the digital precoder and digital combiner at $(i)$.

Let $t$ be the iteration index. 

We initialize $\prebb\node{i}(0)$ and $\combb\node{i}(0)$ as the digital result of hybrid decomposition of the eigen-beamformers of their respective channels.

We first solve for the baseband precoder that maximizes the sum rate.
\begin{align}
\prebb\node{i}(t+1) =& \arg \max_{\prebb} \left\{ \ R_{ij}\left(\prebb\node{i}\right) + R_{ki}\left(\prebb\node{i},\combb\node{i}(t)\right) \right\} \\
&\st \ \frobeniustwo{\prebb\node{i}} \leq \Ns \Nt
\end{align}

Using this choice of $\prebb\node{i}(t+1)$, we solve for the baseband combiner that maximizes the sum rate.
\begin{align}
\combb\node{i}(t+1) =& \arg \max_{\combb} \left\{ \ R_{ij}\left(\prebb\node{i}(t+1)\right) + R_{ki}\left(\prebb\node{i}(t+1),\combb\node{i}\right) \right\} 
% \\ &\st \ \frobeniustwo{\prebb\node{i}} = \Ns \Nt
\end{align}
We iterate between these for a maximum number of iterations or until a convergence criterion is met.

\newpage

Grouping constant terms, we define
\begin{align}
\mat{A} &= \com\ctransnode{j} \channel_{ij} \prerf\node{i} \\
\mat{B} &= \left( \com\ctransnode{j} \mat{R_n} \com\node{j} \right)^{-1}
\end{align}
This gives us the simplified expression
\begin{align}
R_{ij}\left(\prebb\node{i}\right) = \log_2 \left| \mat{I} + \mat{A} \prebb\node{i} \mat{R_s} \prebb\ctransnode{i} \mat{A}\ctrans \mat{B} \right|
\end{align}

Similarly, grouping constant terms, we define
\begin{align}
\mat{C} &= \comrf\ctransnode{i} \channel_{ki} \pre\node{k} \mat{R_s} \pre\ctransnode{k} \channel_{ki}\ctrans \comrf\node{i} \\
\mat{D} &= \channel_{ii} \prerf\node{i}
\end{align}
This gives us the simplified expression 
\begin{align}
R_{ki}\left(\prebb\node{i},\combb\node{i}\right) =& \log_2 \Bigg| \mat{I} + \combb\ctransnode{i} \mat{C} \combb\node{i} \left( \combb\ctransnode{i} \comrf\ctransnode{i} \left( \mat{R_n} + \mat{D} \prebb\node{i} \mat{R_s}  \prebb\ctransnode{i} \mat{D}\ctrans \right) \comrf\node{i} \combb\node{i} \right)^{-1} \Bigg|
\end{align}

\newpage
